Formalizing Data Deletion in the Context of the Right to be Forgotten

The right of an individual to request the deletion of their personal data by an entity that might be storing it -- referred to as the right to be forgotten -- has been explicitly recognized, legislated, and exercised in several jurisdictions across the world, including the European Union, Argentina, and California. However, much of the discussion surrounding this right offers only an intuitive notion of what it means for it to be fulfilled -- of what it means for such personal data to be deleted. In this work, we provide a formal definitional framework for the right to be forgotten using tools and paradigms from cryptography. In particular, we provide a precise definition of what could be (or should be) expected from an entity that collects individuals' data when a request is made of it to delete some of this data. Our framework captures several, though not all, relevant aspects of typical systems involved in data processing. While it cannot be viewed as expressing the statements of current laws (especially since these are rather vague in this respect), our work offers technically precise definitions that represent possibilities for what the law could reasonably expect, and alternatives for what future versions of the law could explicitly require. Finally, with the goal of demonstrating the applicability of our framework and definitions, we consider various natural and simple scenarios where the right to be forgotten comes up. For each of these scenarios, we highlight the pitfalls that arise even in genuine attempts at implementing systems offering deletion guarantees, and also describe technological solutions that provably satisfy our definitions. These solutions bring together techniques built by various communities.

==> notes.tex <==
\section{Notes}
\label{sec:notes}

\begin{itemize}
  \item The parts of the laws that are most relevant to our work are Article 7 (consent and the right to withdraw) and Article 17 (the right to be forgotten) of the GDPR, and 1798.105 in the CCPA, the last of which seems to be the closest to our modelling.
    \begin{itemize}
      \item The GDPR also says, ``The withdrawal of consent shall not affect the lawfulness of processing based on consent before its withdrawal.'' How does this square with our consideration of the whole state of $X$ as opposed to something like just its ``database''?
    \end{itemize}
    \item Whether the definition allows sharing of data between parties? To be compliant, you could not send the private data to other parties. 
    \item Don't need to deal with implementation details - how organization keeps track of who the data belongs to?
    \item It should be okay if I gave my phone number to someone and they store it on their google account. 
    
    \item I posted something on Facebook which was later deleted. In the meantime, someone saved it.
    
    \item allow both way communication between Z and U, this is most restrictive. 
    
    Under this definition you can only get public functions of your private data. 
    
    AWS probably can follow this definition. 
    
    \item definition, compliance, level-0, level-1, level-t
    
    \item is the definition closed under union?
    
    \item attack with the random string.. secret sharing .. so joint distribution is important
    
    \item recursion in the compliance definition seems inherent... one can think of the example where google asks fb to store some data which fb then sends back to google and then google sends it back to fb. 
    
    \item legitimate reasons to remember someone:- fair free trials
    
    \item Decouple why some data is stored from our definitions; for example, another user asks me to store my phone number
    \item Decouple how information is stored. 
    
    \item Small startup can be compliant while storing data on AWS... by just storing keys and (a tree of keys) -- oram issues -- weAKER DEFINITION MIGHT BE FINE... smaller companies could have lower compliance requirements
    
    \item This paper does not interpret the law but provides possible ways to interpret it. 
      Note: Saying something like this is perhaps not the best idea. It sounds like we were being lazy. Perhaps it would be a good idea to read GDPR part on this, along with the interpretation and perhaps say what we think the language of the law asks for. What we think is too restrictive and what else is to libral.

    \item Can we say neural networks forget in some sense? That is, say the entity takes the data it receives, uses it to train a neural net and then discards it. Is any further processing necessary for deletion? I believe there is some work showing that neural networks actually memorise some part of the training data, perhaps that says this isn't sufficient. On the other hand, if each user's data comes from the same distribution, then maybe we can say that each user's data is forgotten with some probability if the storage is not big enough to hold everything. How good is something like this?

    \item Should show that the deletion in ML from the talk satisfies some of our definitions. Should look into existing systems and see whether they fit, for instance Encore.

    \item Look up history-independent data structures and possible connections.

    \item From panel on computation and law: One important use of the right to be forgotten is to enable people to move on. Crimes in the past that have been adequately punished should not unnecessarily influence people's futures.

    \item Should point out the ways in which our definitions are different from privacy requirements (they also talk about their relation to privacy in their Appendix A). And how it relates to the deletion in ML thing.

    \item Should point out that our work is not about determining when deletion is appropriate. Our definition comes in only after it has been decided that somehting has to be deleted. Lawyers seem to find the former a lot more interesting and assume that is what we do, so we should be clear about this.

    \item Address somewhere also why using statistical distance is good enough for us but not for DP. There, they are comparing a database with a given row and a database without it. We are comparing the state when the given row was inserted and deleted, and when it was never inserted in the first place. In particular, it is possible to get perfect compliance in many cases without losing utility.
\end{itemize}

% \noindent Plans:
% \begin{itemize}
%   \item If you collect data, use it to train some ML model, say by linear regression, and then throw away the data, then there is no need to do anything to be compliant as long as the model is much smaller than all the data put together and each user's data comes from the same distribution.
%   \item If you do this but keep the data and then delete the data when asked to but don't update the model, then in the worst-case you are not compliant.
%   \item If you keep the data but do proper ML-deletion things (according to the definition from the video), then also you are compliant.
%   \item If the data collector is, say, publishing some information about the data in public, and this publication is differentially private with respect to the view of the collector, then this should be compliant.
%   \item Can we say that compliance implies some kind of differential privacy? There is some discrepancy in the specifics, but something similar might be true.
%   \item History-independent data structures.
% \end{itemize}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:
